The faint radio sky: VLBA observations of the COSMOS field

We study the faint radio population using wide-field very long baseline interferometry (VLBI) observations of 2865 known radio sources in the Cosmic Evolution Survey (COSMOS) field. The main objective of the project was to determine where active galactic nuclei (AGN) are present. The combination of number of sources, sensitivity, angular resolution and area covered by this project are unprecedented. We have detected 468 radio sources, expected to be AGNs, with the Very Long Baseline Array (VLBA) at 1.4 GHz. This is, to date, the largest sample assembled of VLBI detected sources in the sub-mJy regime. The input sample was taken from previous observations with the Very Large Array (VLA). We present the catalogue with additional multiwavelength information. We find a detection fraction of 20%, considering only those sources from the input catalogue which were in principle detectable with the VLBA (2361). As a function of redshift, we see no evolution of the detection fraction over the redshift range 0.5<z<3. In addition, we find that faint radio sources typically have a greater fraction of their radio luminosity in a compact core: ~70% of the sub-mJy sources detected with the VLBA have more than half of their total radio luminosity in a VLBI-scale component, whereas this is true for only ~30% of the sources that are brighter than 10 mJy. This suggests that fainter radio sources differ intrinsically from brighter ones. Across our entire sample, we find the predominant morphological classification of the host galaxies of the VLBA detected sources to be early type (57%), although this varies with redshift and at z>1.5 we find that spiral galaxies become the most prevalent (48%). We demonstrate that wide-field VLBI observations, together with new calibration methods such as multi-source self-calibration and mosaicing, result in information which is difficult or impossible to obtain otherwise.

==> references <==
@ARTICLE{appleton2004,
   author = {{Appleton}, P.~N. and {Fadda}, D.~T. and {Marleau}, F.~R. and others},
    title = {},
  journal = {\apjs},
   eprint = {astro-ph/0406030},
 keywords = {Cosmology: Observations, Galaxies: Evolution, Galaxies: High-Redshift, Infrared: Galaxies},
     year = 2004,
    month = sep,
   volume = 154,
    pages = {147-150},
      doi = {10.1086/422425},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJS..154..147A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{astropy2013,
   author = {{Astropy Collaboration} and {Robitaille}, T.~P. and {Tollerud}, E.~J. and 
	{Greenfield}, P. and others},
    title = {},
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1307.6212},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, methods: miscellaneous, virtual observatory tools},
     year = 2013,
    month = oct,
   volume = 558,
      eid = {A33},
    pages = {A33},
      doi = {10.1051/0004-6361/201322068},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...558A..33A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{baldi2013,
   author = {{Baldi}, R.~D. and {Chiaberge}, M. and {Capetti}, A. and others},
    title = {},
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1210.4540},
 keywords = {galaxies: active, galaxies: evolution, galaxies: high-redshift, galaxies: nuclei, galaxies: photometry, infrared: galaxies},
     year = 2013,
    month = jan,
   volume = 762,
      eid = {30},
    pages = {30},
      doi = {10.1088/0004-637X/762/1/30},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...762...30B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{baldi2014,
   author = {{Baldi}, R.~D. and {Capetti}, A. and {Chiaberge}, M. and {Celotti}, A.
	},
    title = {},
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1405.1711},
 keywords = {galaxies: active, galaxies: high-redshift, galaxies: jets, galaxies: nuclei, galaxies: photometry},
     year = 2014,
    month = jul,
   volume = 567,
      eid = {A76},
    pages = {A76},
      doi = {10.1051/0004-6361/201423906},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...567A..76B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{bertoldi2007,
   author = {{Bertoldi}, F. and {Carilli}, C. and {Aravena}, M. and others},
    title = {},
  journal = {\apjs},
 keywords = {Submillimeter, Infrared: Galaxies, Surveys},
     year = 2007,
    month = sep,
   volume = 172,
    pages = {132-149},
      doi = {10.1086/520511},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..172..132B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{best2006,
   author = {{Best}, P.~N. and {Kaiser}, C.~R. and {Heckman}, T.~M. and {Kauffmann}, G.
	},
    title = {},
  journal = {\mnras},
   eprint = {astro-ph/0602171},
 keywords = {galaxies: active, galaxies: evolution, galaxies: stellar content, accretion, radio continuum: galaxies},
     year = 2006,
    month = may,
   volume = 368,
    pages = {L67-L71},
      doi = {10.1111/j.1745-3933.2006.00159.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.368L..67B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{best2014,
   author = {{Best}, P.~N. and {Ker}, L.~M. and {Simpson}, C. and others},
    title = {},
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1409.0263},
 keywords = {accretion, accretion discs, galaxies: active, galaxies: evolution, galaxies: jets, radio continuum: galaxies},
     year = 2014,
    month = nov,
   volume = 445,
    pages = {955-969},
      doi = {10.1093/mnras/stu1776},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.445..955B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bonzini2013,
   author = {{Bonzini}, M. and {Padovani}, P. and {Mainieri}, V. and others},
    title = {},
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1310.1248},
 keywords = {catalogues, galaxies: active, galaxies: star formation},
     year = 2013,
    month = dec,
   volume = 436,
    pages = {3759-3771},
      doi = {10.1093/mnras/stt1879},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.436.3759B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{bower2006,
   author = {{Bower}, R.~G. and {Benson}, A.~J. and {Malbon}, R. and others},
    title = {},
  journal = {\mnras},
   eprint = {astro-ph/0511338},
 keywords = {galaxies: evolution: galaxies: formation: galaxies: luminosity function, galaxies: evolution, galaxies: formation, galaxies: luminosity function},
     year = 2006,
    month = aug,
   volume = 370,
    pages = {645-655},
      doi = {10.1111/j.1365-2966.2006.10519.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.370..645B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{boyle2007,
   author = {{Boyle}, B.~J. and {Cornwell}, T.~J. and {Middelberg}, E. and others},
    title = {},
  journal = {\mnras},
   eprint = {astro-ph/0701602},
 keywords = {galaxies: starburst , infrared: galaxies , radio continuum: general},
     year = 2007,
    month = apr,
   volume = 376,
    pages = {1182-1188},
      doi = {10.1111/j.1365-2966.2007.11509.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.376.1182B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{brandt2005,
   author = {{Brandt}, W.~N. and {Hasinger}, G.},
    title = {},
  journal = {\araa},
   eprint = {astro-ph/0501058},
     year = 2005,
    month = sep,
   volume = 43,
    pages = {827-859},
      doi = {10.1146/annurev.astro.43.051804.102213},
   adsurl = {http://adsabs.harvard.edu/abs/2005ARA%26A..43..827B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{brusa2010,
   author = {{Brusa}, M. and {Civano}, F. and {Comastri}, A. and others},
    title = {},
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1004.2790},
 keywords = {galaxies: active, surveys, X-rays: diffuse background, X-rays: galaxies, X-rays: general},
     year = 2010,
    month = jun,
   volume = 716,
    pages = {348-369},
      doi = {10.1088/0004-637X/716/1/348},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...716..348B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cameron2011,
   author = {{Cameron}, E.},
    title = {},
  journal = {\pasa},
archivePrefix = "arXiv",
   eprint = {1012.0566},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, methods: statistical,},
     year = 2011,
    month = jun,
   volume = 28,
    pages = {128-139},
      doi = {10.1071/AS10046},
   adsurl = {http://adsabs.harvard.edu/abs/2011PASA...28..128C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{capak2007,
   author = {{Capak}, P. and {Aussel}, H. and {Ajiki}, M. and others},
    title = {},
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {0704.2430},
 keywords = {Cosmology: Observations, Galaxies: Evolution, Cosmology: Large-Scale Structure of Universe, Surveys},
     year = 2007,
    month = sep,
   volume = 172,
    pages = {99-116},
      doi = {10.1086/519081},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..172...99C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{cappelluti2009,
   author = {{Cappelluti}, N. and {Brusa}, M. and {Hasinger}, G. and others},
    title = {},
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0901.2347},
 primaryClass = "astro-ph.HE",
 keywords = {galaxies: active, large-scale structure of Universe, X-rays: diffuse background, X-rays: galaxies},
     year = 2009,
    month = apr,
   volume = 497,
    pages = {635-648},
      doi = {10.1051/0004-6361/200810794},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...497..635C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{chandra2012,
   author = {{Chandra}, P. and {Frail}, D.~A.},
    title = {},
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1110.4124},
 primaryClass = "astro-ph.CO",
 keywords = {cosmology: observations, gamma-ray burst: general, hydrodynamics, radio continuum: general},
     year = 2012,
    month = feb,
   volume = 746,
      eid = {156},
    pages = {156},
      doi = {10.1088/0004-637X/746/2/156},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...746..156C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{chi2013,
   author = {{Chi}, S. and {Barthel}, P.~D. and {Garrett}, M.~A.},
    title = {},
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1301.1253},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: active, radio continuum: galaxies, galaxies: starburst},
     year = 2013,
    month = feb,
   volume = 550,
      eid = {A68},
    pages = {A68},
      doi = {10.1051/0004-6361/201220783},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...550A..68C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{civano2012,
   author = {{Civano}, F. and {Elvis}, M. and {Brusa}, M. and others},
    title = {},
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1205.5030},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: active, surveys, X-rays: galaxies: clusters},
     year = 2012,
    month = aug,
   volume = 201,
      eid = {30},
    pages = {30},
      doi = {10.1088/0067-0049/201/2/30},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJS..201...30C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{civano2016,
   author = {{Civano}, F. and {Marchesi}, S. and {Comastri}, A. and others},
    title = {},
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1601.00941},
 keywords = {catalogs, cosmology: observations, galaxies: evolution, quasars: general, surveys, X-rays: general},
     year = 2016,
    month = mar,
   volume = 819,
      eid = {62},
    pages = {62},
      doi = {10.3847/0004-637X/819/1/62},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...819...62C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{condon1992,
   author = {{Condon}, J.~J.},
    title = {},
  journal = {\araa},
 keywords = {Cosmic Rays, Radio Emission, Radio Sources (Astronomy), Star Formation, Starburst Galaxies, Synchrotron Radiation, Black Holes (Astronomy), H Ii Regions, Infrared Radiation, Relativistic Particles},
     year = 1992,
   volume = 30,
    pages = {575-611},
      doi = {10.1146/annurev.aa.30.090192.003043},
   adsurl = {http://adsabs.harvard.edu/abs/1992ARA%26A..30..575C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{croton2006,
   author = {{Croton}, D.~J. and {Springel}, V. and {White}, S.~D.~M. and 
	others},
    title = {},
  journal = {\mnras},
   eprint = {astro-ph/0508046},
 keywords = {black hole physics, galaxies: active, cooling flows, galaxies: evolution, galaxies: formation, cosmology: theory},
     year = 2006,
    month = jan,
   volume = 365,
    pages = {11-28},
      doi = {10.1111/j.1365-2966.2005.09675.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.365...11C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{deller2007,
   author = {{Deller}, A.~T. and {Tingay}, S.~J. and {Bailes}, M. and {West}, C.
	},
    title = {},
  journal = {\pasp},
   eprint = {astro-ph/0702141},
 keywords = {Techniques: Interferometric, Instrumentation: Interferometers, Stars: Pulsars: General, Radio Continuum: General, Radio Lines: General},
     year = 2007,
    month = mar,
   volume = 119,
    pages = {318-336},
      doi = {10.1086/513572},
   adsurl = {http://adsabs.harvard.edu/abs/2007PASP..119..318D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{deller2011,
   author = {{Deller}, A.~T. and {Brisken}, W.~F. and {Phillips}, C.~J. and 
	others
	},
    title = {},
  journal = {\pasp},
archivePrefix = "arXiv",
   eprint = {1101.0885},
 primaryClass = "astro-ph.IM",
 keywords = {Astronomical Instrumentation},
     year = 2011,
    month = mar,
   volume = 123,
    pages = {275-287},
      doi = {10.1086/658907},
   adsurl = {http://adsabs.harvard.edu/abs/2011PASP..123..275D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{deller2014,
   author = {{Deller}, A.~T. and {Middelberg}, E.},
    title = {},
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1310.8191},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: active, radio continuum: galaxies, surveys, techniques: high angular resolution, techniques: interferometric},
     year = 2014,
    month = jan,
   volume = 147,
      eid = {14},
    pages = {14},
      doi = {10.1088/0004-6256/147/1/14},
   adsurl = {http://adsabs.harvard.edu/abs/2014AJ....147...14D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{deller2016,
   author = {{Deller}, A.~T. and {Vigeland}, S.~J. and {Kaplan}, D.~L. and others},
    title = {},
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1604.02367},
 primaryClass = "astro-ph.SR",
 keywords = {astrometry, pulsars: individual: PSR J1022+1001, J2145{\ndash}0750, stars: neutron, techniques: high angular resolution, white dwarfs},
     year = 2016,
    month = sep,
   volume = 828,
      eid = {8},
    pages = {8},
      doi = {10.3847/0004-637X/828/1/8},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...828....8D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{delvecchio2017,
   author = {{Delvecchio}, I. and {Smol{\v c}i{\'c}}, V. and {Zamorani}, G. and others},
    title = {},
  journal = {ArXiv:1703.09720},
archivePrefix = "arXiv",
   eprint = {1703.09720},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2017,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170309720D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{dubois2013,
   author = {{Dubois}, Y. and {Gavazzi}, R. and {Peirani}, S. and {Silk}, J.
	},
    title = {},
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1301.3092},
 primaryClass = "astro-ph.CO",
 keywords = {methods: numerical, galaxies: active, galaxies: elliptical and lenticular, cD, galaxies: formation, galaxies: jets, galaxies: kinematics and dynamics},
     year = 2013,
    month = aug,
   volume = 433,
    pages = {3297-3313},
      doi = {10.1093/mnras/stt997},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.433.3297D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{fomalont1981,
   author = {{Fomalont}, E.},
    title = {},
  journal = {National Radio Astronomy Observatory Newsletter},
     year = 1981,
   volume = 3,
    pages = {3},
   adsurl = {http://adsabs.harvard.edu/abs/1981NRAON...3....3F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{frayer2009,
   author = {{Frayer}, D.~T. and {Sanders}, D.~B. and {Surace}, J.~A. and 
	others
	},
    title = {},
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {0902.3273},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: evolution, galaxies: starburst, infrared: galaxies},
     year = 2009,
    month = nov,
   volume = 138,
    pages = {1261-1270},
      doi = {10.1088/0004-6256/138/5/1261},
   adsurl = {http://adsabs.harvard.edu/abs/2009AJ....138.1261F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gabor2009,
   author = {{Gabor}, J.~M. and {Impey}, C.~D. and {Jahnke}, K. and others},
    title = {},
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0809.0309},
 keywords = {galaxies: active, galaxies: evolution, galaxies: interactions, galaxies: structure},
     year = 2009,
    month = jan,
   volume = 691,
    pages = {705-722},
      doi = {10.1088/0004-637X/691/1/705},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...691..705G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{gaibler2012,
   author = {{Gaibler}, V. and {Khochfar}, S. and {Krause}, M. and {Silk}, J.
	},
    title = {},
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1111.4478},
 primaryClass = "astro-ph.CO",
 keywords = {hydrodynamics, methods: numerical, ISM: clouds, galaxies: jets, galaxies: ISM, galaxies: star formation },
     year = 2012,
    month = sep,
   volume = 425,
    pages = {438-449},
      doi = {10.1111/j.1365-2966.2012.21479.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.425..438G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{garrett1999,
   author = {{Garrett}, M.~A. and {Porcas}, R.~W. and {Pedlar}, A. and {Muxlow}, T.~W.~B. and 
	{Garrington}, S.~T.},
    title = {},
  journal = {\nar},
   eprint = {astro-ph/9906108},
     year = 1999,
    month = nov,
   volume = 43,
    pages = {519-522},
      doi = {10.1016/S1387-6473(99)00045-7},
   adsurl = {http://adsabs.harvard.edu/abs/1999NewAR..43..519G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{garrett2001,
   author = {{Garrett}, M.~A. and {Muxlow}, T.~W.~B. and {Garrington}, S.~T. and others},
    title = {},
  journal = {\aap},
   eprint = {astro-ph/0102037},
 keywords = {GALAXIES: ACTIVE, GALAXIES: RADIO CONTINUUM, GALAXIES: STARBURST},
     year = 2001,
    month = feb,
   volume = 366,
    pages = {L5-L8},
      doi = {10.1051/0004-6361:20000537},
   adsurl = {http://adsabs.harvard.edu/abs/2001A%26A...366L...5G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{garrett2005,
   author = {{Garrett}, M.~A. and {Wrobel}, J.~M. and {Morganti}, R.},
    title = {},
  journal = {\apj},
   eprint = {astro-ph/0410176},
 keywords = {Galaxies: Active, Galaxies: Starburst, Radio Continuum: Galaxies, Surveys, Techniques: Interferometric},
     year = 2005,
    month = jan,
   volume = 619,
    pages = {105-115},
      doi = {10.1086/426424},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...619..105G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{giroletti2009,
   author = {{Giroletti}, M. and {Panessa}, F.},
    title = {},
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0910.5821},
 keywords = {galaxies: active, galaxies: Seyfert, radio continuum: galaxies},
     year = 2009,
    month = dec,
   volume = 706,
    pages = {L260-L264},
      doi = {10.1088/0004-637X/706/2/L260},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...706L.260G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{greisen2003,
   author = {{Greisen}, E.~W.},
    title = {},
  journal = {Information Handling in Astronomy - Historical Vistas},
     year = 2003,
    month = mar,
   volume = 285,
    pages = {109},
      doi = {10.1007/0-306-48080-8_7},
   adsurl = {http://adsabs.harvard.edu/abs/2003ASSL..285..109G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{hales2012,
   author = {{Hales}, C.~A. and {Murphy}, T. and {Curran}, J.~R. and others},
    title = {},
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1205.5313},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, methods: statistical, techniques: image processing, techniques: polarimetric Surveys, catalogues, surveys },
     year = 2012,
    month = sep,
   volume = 425,
    pages = {979-996},
      doi = {10.1111/j.1365-2966.2012.21373.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.425..979H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hales2014,
   author = {{Hales}, C.~A. and {Norris}, R.~P. and {Gaensler}, B.~M. and others},
    title = {},
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1403.5307},
 primaryClass = "astro-ph.GA",
 keywords = {polarization, methods: data analysis, techniques: polarimetric, surveys, radio continuum: galaxies},
     year = 2014,
    month = jul,
   volume = 441,
    pages = {2555-2592},
      doi = {10.1093/mnras/stu576},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.441.2555H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{hao2014,
   author = {{Hao}, H. and {Elvis}, M. and {Civano}, F. and others},
    title = {},
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1210.3033},
 primaryClass = "astro-ph.GA",
 keywords = {surveys, galaxies: evolution, quasars: general},
     year = 2014,
    month = feb,
   volume = 438,
    pages = {1288-1304},
      doi = {10.1093/mnras/stt2274},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.438.1288H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hardcastle2006,
   author = {{Hardcastle}, M.~J. and {Evans}, D.~A. and {Croston}, J.~H.},
    title = {},
  journal = {\mnras},
   eprint = {astro-ph/0603090},
 keywords = {galaxies: active: X-rays: galaxies, galaxies: active, X-rays: galaxies},
     year = 2006,
    month = aug,
   volume = 370,
    pages = {1893-1904},
      doi = {10.1111/j.1365-2966.2006.10615.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.370.1893H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{hasinger2007,
   author = {{Hasinger}, G. and {Cappelluti}, N. and {Brunner}, H. and others},
    title = {},
  journal = {\apjs},
   eprint = {astro-ph/0612311},
 keywords = {Cosmology: Observations, Cosmology: Large-Scale Structure of Universe, Cosmology: Dark Matter, Galaxies: Formation, Galaxies: Evolution, X-Rays: Galaxies},
     year = 2007,
    month = sep,
   volume = 172,
    pages = {29-37},
      doi = {10.1086/516576},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..172...29H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{heckman2014,
   author = {{Heckman}, T.~M. and {Best}, P.~N.},
    title = {},
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {1403.4620},
 primaryClass = "astro-ph.GA",
     year = 2014,
    month = aug,
   volume = 52,
    pages = {589-660},
      doi = {10.1146/annurev-astro-081913-035722},
   adsurl = {http://adsabs.harvard.edu/abs/2014ARA%26A..52..589H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{herreraruiz2016,
   author = {{Herrera Ruiz}, N. and {Middelberg}, E. and {Norris}, R.~P. and 
	{Maini}, A.},
    title = {},
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1603.07136},
 keywords = {galaxies: active, radio continuum: galaxies, quasars: general, galaxies: evolution},
     year = 2016,
    month = may,
   volume = 589,
      eid = {L2},
    pages = {L2},
      doi = {10.1051/0004-6361/201628302},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...589L...2H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{ishibashi2012,
   author = {{Ishibashi}, W. and {Fabian}, A.~C.},
    title = {},
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1209.1480},
 primaryClass = "astro-ph.GA",
 keywords = {black hole physics, stars: formation, galaxies: active, galaxies: evolution},
     year = 2012,
    month = dec,
   volume = 427,
    pages = {2998-3005},
      doi = {10.1111/j.1365-2966.2012.22074.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.427.2998I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kartaltepe2010,
   author = {{Kartaltepe}, J.~S. and {Sanders}, D.~B. and {Le Floc'h}, E. and 
	others},
    title = {},
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0911.4515},
 keywords = {cosmology: observations, galaxies: active, galaxies: evolution, galaxies: high-redshift, infrared: galaxies, surveys},
     year = 2010,
    month = feb,
   volume = 709,
    pages = {572-596},
      doi = {10.1088/0004-637X/709/2/572},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...709..572K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kartaltepe2010b,
   author = {{Kartaltepe}, J.~S. and {Sanders}, D.~B. and {Le Floc'h}, E. and 
	others},
    title = {},
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1006.4956},
 keywords = {cosmology: observations, galaxies: active, galaxies: evolution, galaxies: high-redshift, infrared: galaxies, surveys},
     year = 2010,
    month = sep,
   volume = 721,
    pages = {98-123},
      doi = {10.1088/0004-637X/721/1/98},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...721...98K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{kettenis2006,
   author = {{Kettenis}, M. and {van Langevelde}, H.~J. and {Reynolds}, C. and 
	{Cotton}, B.},
    title = {},
booktitle = {Astronomical Data Analysis Software and Systems XV},
     year = 2006,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 351,
   editor = {{Gabriel}, C. and {Arviset}, C. and {Ponz}, D. and {Enrique}, S.
	},
    month = jul,
    pages = {497},
   adsurl = {http://adsabs.harvard.edu/abs/2006ASPC..351..497K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{kewley2000,
   author = {{Kewley}, L.~J. and {Heisler}, C.~A. and {Dopita}, M.~A. and 
	others},
    title = {},
  journal = {\apj},
 keywords = {GALAXIES: ACTIVE, INFRARED: GALAXIES, RADIO CONTINUUM: GALAXIES},
     year = 2000,
    month = feb,
   volume = 530,
    pages = {704-718},
      doi = {10.1086/308397},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...530..704K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lackner2014,
   author = {{Lackner}, C.~N. and {Silverman}, J.~D. and {Salvato}, M. and 
	others},
    title = {},
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1406.2327},
 keywords = {galaxies: active, galaxies: formation, galaxies: interactions, techniques: image processing},
     year = 2014,
    month = dec,
   volume = 148,
      eid = {137},
    pages = {137},
      doi = {10.1088/0004-6256/148/6/137},
   adsurl = {http://adsabs.harvard.edu/abs/2014AJ....148..137L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lanzuisi2015,
   author = {{Lanzuisi}, G. and {Ranalli}, P. and {Georgantopoulos}, I. and others},
    title = {},
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1409.1867},
 keywords = {galaxies: nuclei, galaxies: Seyfert, quasars: general, X-rays: galaxies},
     year = 2015,
    month = jan,
   volume = 573,
      eid = {A137},
    pages = {A137},
      doi = {10.1051/0004-6361/201424924},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...573A.137L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{lenc2008,
   author = {{Lenc}, E. and {Garrett}, M.~A. and {Wucknitz}, O. and {Anderson}, J.~M. and 
	{Tingay}, S.~J.},
    title = {},
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0710.1946},
 keywords = {galaxies: active, quasars: individual: QSO B0218+357 J0226+3421, radiation mechanisms: general, techniques: interferometric},
     year = 2008,
    month = jan,
   volume = 673,
      eid = {78-95},
    pages = {78-95},
      doi = {10.1086/524295},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...673...78L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lien2011,
   author = {{Lien}, A. and {Chakraborty}, N. and {Fields}, B.~D. and {Kemball}, A.
	},
    title = {},
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1107.0775},
 primaryClass = "astro-ph.CO",
 keywords = {radio continuum: stars, supernovae: general, surveys},
     year = 2011,
    month = oct,
   volume = 740,
      eid = {23},
    pages = {23},
      doi = {10.1088/0004-637X/740/1/23},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...740...23L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lilly2007,
   author = {{Lilly}, S.~J. and {Le F{\`e}vre}, O. and {Renzini}, A. and 
	others},
    title = {},
  journal = {\apjs},
   eprint = {astro-ph/0612291},
 keywords = {Cosmology: Observations, Galaxies: Active, Galaxies: Distances and Redshifts, Galaxies: Evolution, Cosmology: Large-Scale Structure of Universe, Galaxies: Quasars: General, Surveys},
     year = 2007,
    month = sep,
   volume = 172,
    pages = {70-85},
      doi = {10.1086/516589},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..172...70L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lusso2011,
   author = {{Lusso}, E. and {Comastri}, A. and {Vignali}, C. and others},
    title = {},
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1108.4925},
 primaryClass = "astro-ph.CO",
 keywords = {methods: statistical, quasars: general, galaxies: active, Galaxy: general, X-rays: general},
     year = 2011,
    month = oct,
   volume = 534,
      eid = {A110},
    pages = {A110},
      doi = {10.1051/0004-6361/201117175},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...534A.110L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{maini2016,
   author = {{Maini}, A. and {Prandoni}, I. and {Norris}, R.~P. and others},
    title = {},
  journal = {\aap},
 keywords = {galaxies: active, galaxies: high-redshift, radio continuum: galaxies},
     year = 2016,
    month = may,
   volume = 589,
      eid = {L3},
    pages = {L3},
      doi = {10.1051/0004-6361/201628305},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...589L...3M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{middelberg2006,
   author = {{Middelberg}, E.},
    title = {},
  journal = {\pasa},
   eprint = {astro-ph/0603216},
 keywords = {Keywords methods: data analysis,},
     year = 2006,
    month = may,
   volume = 23,
    pages = {64-68},
      doi = {10.1071/AS06004},
   adsurl = {http://adsabs.harvard.edu/abs/2006PASA...23...64M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{middelberg2010,
   author = {{Middelberg}, E. and {Deller}, A. and {Morgan}, J. and others},
    title = {},
booktitle = {10th European VLBI Network Symposium and EVN Users Meeting: VLBI and the New Generation of Radio Arrays},
     year = 2010,
archivePrefix = "arXiv",
   eprint = {1011.2404},
 primaryClass = "astro-ph.CO",
      eid = {26},
    pages = {26},
   adsurl = {http://adsabs.harvard.edu/abs/2010evn..confE..26M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{middelberg2011,
   author = {{Middelberg}, E. and {Deller}, A. and {Morgan}, J. and others},
    title = {},
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1011.2400},
 primaryClass = "astro-ph.CO",
 keywords = {techniques: interferometric, galaxies: active, galaxies: evolution},
     year = 2011,
    month = feb,
   volume = 526,
      eid = {A74},
    pages = {A74},
      doi = {10.1051/0004-6361/201015406},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...526A..74M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{middelberg2013,
   author = {{Middelberg}, E. and {Deller}, A.~T. and {Norris}, R.~P. and 
	others},
    title = {},
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1212.4605},
 primaryClass = "astro-ph.CO",
 keywords = {techniques: interferometric, galaxies: active, galaxies: evolution},
     year = 2013,
    month = mar,
   volume = 551,
      eid = {A97},
    pages = {A97},
      doi = {10.1051/0004-6361/201220374},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...551A..97M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{moric2010,
   author = {{Mori{\'c}}, I. and {Smol{\v c}i{\'c}}, V. and {Kimball}, A. and 
	others
	},
    title = {},
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1010.0435},
 primaryClass = "astro-ph.GA",
 keywords = {cosmology: observations, evolution, galaxies: active, galaxies: fundamental parameters, radio continuum: galaxies},
     year = 2010,
    month = nov,
   volume = 724,
    pages = {779-790},
      doi = {10.1088/0004-637X/724/1/779},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...724..779M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{mullin2008,
   author = {{Mullin}, L.~M. and {Riley}, J.~M. and {Hardcastle}, M.~J.},
    title = {},
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0806.1313},
 keywords = {galaxies: active , galaxies: jets , radio continuum: galaxies},
     year = 2008,
    month = oct,
   volume = 390,
    pages = {595-621},
      doi = {10.1111/j.1365-2966.2008.13534.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.390..595M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{mushotzky2004,
   author = {{Mushotzky}, R.},
    title = {},
booktitle = {Supermassive Black Holes in the Distant Universe},
     year = 2004,
   series = {Astrophysics and Space Science Library},
   volume = 308,
   eprint = {astro-ph/0405144},
   editor = {{Barger}, A.~J.},
    month = aug,
    pages = {53},
      doi = {10.1007/978-1-4020-2471-9_2},
   adsurl = {http://adsabs.harvard.edu/abs/2004ASSL..308...53M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{nagar2002,
   author = {{Nagar}, N.~M. and {Falcke}, H. and {Wilson}, A.~S. and {Ulvestad}, J.~S.
	},
    title = {},
  journal = {\aap},
   eprint = {astro-ph/0207176},
 keywords = {accretion, accretion disks, galaxies: active, galaxies: jets, galaxies: nuclei, radio continuum: galaxies, surveys},
     year = 2002,
    month = sep,
   volume = 392,
    pages = {53-82},
      doi = {10.1051/0004-6361:20020874},
   adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...392...53N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{norris2009,
   author = {{Norris}, R.~P.},
    title = {},
booktitle = {The Starburst-AGN Connection},
     year = 2009,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 408,
archivePrefix = "arXiv",
   eprint = {0909.3676},
   editor = {{Wang}, W. and {Yang}, Z. and {Luo}, Z. and {Chen}, Z.},
    month = oct,
    pages = {334},
   adsurl = {http://adsabs.harvard.edu/abs/2009ASPC..408..334N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{norris2012,
   author = {{Norris}, R.~P. and {Lenc}, E. and {Roy}, A.~L. and {Spoon}, H.
	},
    title = {},
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1107.3895},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: active, galaxies: evolution, galaxies: jets, radio continuum: galaxies},
     year = 2012,
    month = may,
   volume = 422,
    pages = {1453-1459},
      doi = {10.1111/j.1365-2966.2012.20717.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.422.1453N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{obric2006,
   author = {{Obri{\'c}}, M. and {Ivezi{\'c}}, {\v Z}. and {Best}, P.~N. and others},
    title = {},
  journal = {\mnras},
   eprint = {astro-ph/0606344},
 keywords = {surveys: galaxies: active: galaxies: fundamental parameters: galaxies: starburst: infrared: galaxies: radio continuum: galaxies, surveys, galaxies: active, galaxies: fundamental parameters, galaxies: starburst, infrared: galaxies, radio continuum: galaxies},
     year = 2006,
    month = aug,
   volume = 370,
    pages = {1677-1698},
      doi = {10.1111/j.1365-2966.2006.10675.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.370.1677O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{padovani2011,
   author = {{Padovani}, P. and {Miller}, N. and {Kellermann}, K.~I. and others},
    title = {},
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1107.2759},
 keywords = {galaxies: active, galaxies: starburst, infrared: galaxies, radio continuum: galaxies, X-rays: galaxies},
     year = 2011,
    month = oct,
   volume = 740,
      eid = {20},
    pages = {20},
      doi = {10.1088/0004-637X/740/1/20},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...740...20P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{planck2014,
   author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and 
	{Armitage-Caplan}, C. and others},
    title = {},
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1303.5076},
 primaryClass = "astro-ph.CO",
 keywords = {cosmic background radiation, cosmological parameters, early Universe, inflation, primordial nucleosynthesis},
     year = 2014,
    month = nov,
   volume = 571,
      eid = {A16},
    pages = {A16},
      doi = {10.1051/0004-6361/201321591},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...571A..16P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{prandoni2010,
   author = {{Prandoni}, I. and {de Ruiter}, H.~R. and {Ricci}, R. and others},
    title = {},
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0911.2697},
 keywords = {surveys, radio continuum: general, methods: data analysis, catalogs, galaxies:, general, galaxies: evolution},
     year = 2010,
    month = feb,
   volume = 510,
      eid = {A42},
    pages = {A42},
      doi = {10.1051/0004-6361/200913052},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...510A..42P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{radcliffe2016,
   author = {{Radcliffe}, J.~F. and {Garrett}, M.~A. and {Beswick}, R.~J. and 
	{Muxlow}, T.~W.~B. and {Barthel}, P.~D. and {Deller}, A.~T. and 
	{Middelberg}, E.},
    title = {},
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1601.04452},
 primaryClass = "astro-ph.IM",
 keywords = {techniques: interferometric, radio continuum: galaxies, instrumentation: interferometers},
     year = 2016,
    month = mar,
   volume = 587,
      eid = {A85},
    pages = {A85},
      doi = {10.1051/0004-6361/201527980},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...587A..85R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{ranalli2012,
   author = {{Ranalli}, P. and {Comastri}, A. and {Zamorani}, G. and others},
    title = {},
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1204.4485},
 primaryClass = "astro-ph.CO",
 keywords = {X-rays: galaxies, radio continuum: galaxies, galaxies: fundamental parameters, galaxies: star formation, galaxies: active, galaxies: high-redshift},
     year = 2012,
    month = jun,
   volume = 542,
      eid = {A16},
    pages = {A16},
      doi = {10.1051/0004-6361/201118723},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...542A..16R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{rees2016,
   author = {{Rees}, G.~A. and {Spitler}, L.~R. and {Norris}, R.~P. and others},
    title = {},
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1511.01988},
 keywords = {galaxies: active, galaxies: evolution, galaxies: high-redshift, galaxies: stellar content, infrared: galaxies, radio continuum: galaxies},
     year = 2016,
    month = jan,
   volume = 455,
    pages = {2731-2744},
      doi = {10.1093/mnras/stv2468},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.455.2731R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{rodriguez2006,
   author = {{Rodriguez}, C. and {Taylor}, G.~B. and {Zavala}, R.~T. and others},
    title = {},
  journal = {\apj},
   eprint = {astro-ph/0604042},
 keywords = {Galaxies: Active, Galaxies: Individual: Alphanumeric: 0402+379, Radio Continuum: Galaxies, Radio Lines: Galaxies},
     year = 2006,
    month = jul,
   volume = 646,
    pages = {49-60},
      doi = {10.1086/504825},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...646...49R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{roy1998,
   author = {{Roy}, A.~L. and {Norris}, R.~P. and {Kesteven}, M.~J. and {Troup}, E.~R. and 
	{Reynolds}, J.~E.},
    title = {},
  journal = {\mnras},
 keywords = {GALAXIES: ACTIVE, GALAXIES: NUCLEI, GALAXIES: SEYFERT, GALAXIES: STARBURST, INFRARED: GALAXIES, RADIO CONTINUUM: GALAXIES},
     year = 1998,
    month = dec,
   volume = 301,
    pages = {1019-1030},
      doi = {10.1046/j.1365-8711.1998.02060.x},
   adsurl = {http://adsabs.harvard.edu/abs/1998MNRAS.301.1019R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{salvato2011,
   author = {{Salvato}, M. and {Ilbert}, O. and {Hasinger}, G. and others},
    title = {},
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1108.6061},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: active, galaxies: distances and redshifts, methods: data analysis, surveys, techniques: photometric, X-rays: galaxies},
     year = 2011,
    month = dec,
   volume = 742,
      eid = {61},
    pages = {61},
      doi = {10.1088/0004-637X/742/2/61},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...742...61S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{schawinski2009,
   author = {{Schawinski}, K. and {Lintott}, C.~J. and {Thomas}, D. and others},
    title = {},
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0809.1096},
 keywords = {galaxies: active, galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation},
     year = 2009,
    month = jan,
   volume = 690,
    pages = {1672-1680},
      doi = {10.1088/0004-637X/690/2/1672},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...690.1672S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{schinnerer2007,
   author = {{Schinnerer}, E. and {Smol{\v c}i{\'c}}, V. and {Carilli}, C.~L. and others},
    title = {},
  journal = {\apjs},
   eprint = {astro-ph/0612314},
 keywords = {Cosmology: Observations, Radio Continuum: Galaxies, Surveys},
     year = 2007,
    month = sep,
   volume = 172,
    pages = {46-69},
      doi = {10.1086/516587},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..172...46S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{schinnerer2010,
   author = {{Schinnerer}, E. and {Sargent}, M.~T. and {Bondi}, M. and others},
    title = {},
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1005.1641},
 primaryClass = "astro-ph.CO",
 keywords = {cosmology: observations, radio continuum: galaxies, surveys},
     year = 2010,
    month = jun,
   volume = 188,
    pages = {384-404},
      doi = {10.1088/0067-0049/188/2/384},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJS..188..384S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{scoville2007,
   author = {{Scoville}, N. and {Aussel}, H. and {Brusa}, M. and others},
    title = {},
  journal = {\apjs},
   eprint = {astro-ph/0612305},
 keywords = {Cosmology: Observations, Cosmology: Dark Matter, Galaxies: Evolution, Galaxies: Formation, Cosmology: Large-Scale Structure of Universe, Surveys},
     year = 2007,
    month = sep,
   volume = 172,
    pages = {1-8},
      doi = {10.1086/516585},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..172....1S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{seymour2012,
   author = {{Seymour}, N. and {Altieri}, B. and {De Breuck}, C. and others},
    title = {},
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1206.5821},
 keywords = {galaxies: active, galaxies: formation, galaxies: high-redshift, galaxies: individual: MRC 1138-262},
     year = 2012,
    month = aug,
   volume = 755,
      eid = {146},
    pages = {146},
      doi = {10.1088/0004-637X/755/2/146},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...755..146S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{shepherd1997,
   author = {{Shepherd}, M.~C.},
    title = {},
booktitle = {Astronomical Data Analysis Software and Systems VI},
     year = 1997,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 125,
   editor = {{Hunt}, G. and {Payne}, H.},
    pages = {77},
   adsurl = {http://adsabs.harvard.edu/abs/1997ASPC..125...77S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{smolcic2009,
   author = {{Smol{\v c}i{\'c}}, V. and {Zamorani}, G. and {Schinnerer}, E. and others},
    title = {},
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0901.3372},
 primaryClass = "astro-ph.CO",
 keywords = {cosmology: observations, galaxies: active, galaxies: evolution, galaxies: fundamental parameters, radio continuum: galaxies},
     year = 2009,
    month = may,
   volume = 696,
    pages = {24-39},
      doi = {10.1088/0004-637X/696/1/24},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...696...24S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{smolcic2014,
   author = {{Smol{\v c}i{\'c}}, V. and {Ciliegi}, P. and {Jeli{\'c}}, V. and others},
    title = {},
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1407.4844},
 keywords = {radiation mechanisms: general, surveys, radio continuum: galaxies},
     year = 2014,
    month = sep,
   volume = 443,
    pages = {2590-2598},
      doi = {10.1093/mnras/stu1331},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.443.2590S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{smolcic2017a,
   author = {{Smol{\v c}i{\'c}}, V. and others},
    title = {},
  journal = {ArXiv e-prints [arXiv:1703.09713]},
archivePrefix = "arXiv",
   eprint = {1703.09713},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2017,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170309713S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{smolcic2017,
   author = {{Smol{\v c}i{\'c}}, V. and others},
    title = {},
  journal = {ArXiv e-prints [arXiv:1703.09719]},
archivePrefix = "arXiv",
   eprint = {1703.09719},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2017,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170309719S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{strazzullo2010,
   author = {{Strazzullo}, V. and {Pannella}, M. and {Owen}, F.~N. and others},
    title = {},
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1003.4734},
 primaryClass = "astro-ph.CO",
 keywords = {cosmology: observations, galaxies: active, galaxies: evolution, galaxies: starburst, radio continuum: galaxies},
     year = 2010,
    month = may,
   volume = 714,
    pages = {1305-1323},
      doi = {10.1088/0004-637X/714/2/1305},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...714.1305S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{taniguchi2007,
   author = {{Taniguchi}, Y. and {Scoville}, N. and {Murayama}, T. and others},
    title = {},
  journal = {\apjs},
   eprint = {astro-ph/0612295},
 keywords = {Galaxies: Evolution, Galaxies: Interactions},
     year = 2007,
    month = sep,
   volume = 172,
    pages = {9-28},
      doi = {10.1086/516596},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..172....9T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tasca2009,
   author = {{Tasca}, L.~A.~M. and {Kneib}, J.-P. and {Iovino}, A. and others},
    title = {},
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0906.4556},
 keywords = {galaxies: fundamental parameters, cosmology: large-scale structure of universe, galaxies: distances and redshifts, galaxies: structure, galaxies: evolution, Galaxy: formation},
     year = 2009,
    month = aug,
   volume = 503,
    pages = {379-398},
      doi = {10.1051/0004-6361/200912213},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...503..379T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{taylor2005,
   author = {{Taylor}, M.~B.},
    title = {},
booktitle = {Astronomical Data Analysis Software and Systems XIV},
     year = 2005,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 347,
   editor = {{Shopbell}, P. and {Britton}, M. and {Ebert}, R.},
    month = dec,
    pages = {29},
   adsurl = {http://adsabs.harvard.edu/abs/2005ASPC..347...29T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tinti2006,
   author = {{Tinti}, S. and {de Zotti}, G.},
    title = {},
  journal = {\aap},
   eprint = {astro-ph/0509439},
 keywords = {galaxies: active, radio continuum: galaxies},
     year = 2006,
    month = jan,
   volume = 445,
    pages = {889-899},
      doi = {10.1051/0004-6361:20053752},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...445..889T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{treister2009,
   author = {{Treister}, E. and {Urry}, C.~M. and {Virani}, S.},
    title = {},
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0902.0608},
 keywords = {galaxies: active, galaxies: Seyfert, X-rays: diffuse background, X-rays: galaxies},
     year = 2009,
    month = may,
   volume = 696,
    pages = {110-120},
      doi = {10.1088/0004-637X/696/1/110},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...696..110T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{trump2007,
   author = {{Trump}, J.~R. and {Impey}, C.~D. and {McCarthy}, P.~J. and others},
    title = {},
  journal = {\apjs},
   eprint = {astro-ph/0606016},
 keywords = {Galaxies: Active, Galaxies: Quasars: General, Surveys},
     year = 2007,
    month = sep,
   volume = 172,
    pages = {383-395},
      doi = {10.1086/516578},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..172..383T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{trump2009,
   author = {{Trump}, J.~R. and {Impey}, C.~D. and {Elvis}, M. and others},
    title = {},
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0811.3977},
 keywords = {galaxies: active, galaxies: Seyfert, quasars: general, surveys, X-rays: galaxies},
     year = 2009,
    month = may,
   volume = 696,
    pages = {1195-1212},
      doi = {10.1088/0004-637X/696/2/1195},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...696.1195T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{trump2011,
   author = {{Trump}, J.~R. and {Impey}, C.~D. and {Kelly}, B.~C. and others},
    title = {},
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1103.0276},
 keywords = {accretion, accretion disks, galaxies: active, galaxies: nuclei, galaxies: Seyfert, quasars: emission lines, quasars: general},
     year = 2011,
    month = may,
   volume = 733,
      eid = {60},
    pages = {60},
      doi = {10.1088/0004-637X/733/1/60},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...733...60T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{zinn2013,
   author = {{Zinn}, P.-C. and {Middelberg}, E. and {Norris}, R.~P. and {Dettmar}, R.-J.
	},
    title = {},
  journal = {\apj},
 keywords = {galaxies: active, galaxies: evolution, galaxies: formation, galaxies: jets, galaxies: star formation, ISM: jets and outflows },
     year = 2013,
    month = sep,
   volume = 774,
      eid = {66},
    pages = {66},
      doi = {10.1088/0004-637X/774/1/66},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...774...66Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

